Incremental View Maintenance for Property Graph Queries

This paper discusses the challenges of incremental view maintenance for property graph queries. We select a subset of property graph queries and present an approach that uses nested relational algebra to allow incremental evaluation.

==> listing-grammar.tex <==
\begin{lstlisting}[caption=Grammar specification of the \oci language. Comments and whitespaces are omitted for conciseness.]
Query:       Clause (Clause)*
Clause:      Match | Unwind | Return
Match:       'MATCH' Pattern Where
Unwind:      'UNWIND' Expression 'AS' Variable
Return:      'RETURN' 'DISTINCT'? ReturnBody
ReturnBody:  ReturnItem (',' ReturnItem)* (Order)? (Limit)?
ReturnItem:  Expression ('AS' Variable)?
Order:       'ORDER BY' SortItem (',' SortItem)*
Limit:       'LIMIT' Expression
SortItem:    (Expression ('DESC' | 'ASC')?)
Where:       'WHERE' Expression
Pattern:     PatternPart (',' PatternPart)*
PatternPart:          (Variable '=' PatternElement) | PatternElement
PatternElement:       (NodePattern (PatternElementChain)*) | '(' PatternElement ')'
NodePattern:          '(' Variable? NodeLabels? Properties? ')'
PatternElementChain:  ('<'? '-' RelationshipDetail '-' '>'? ) NodePattern
RelationshipDetail:   '[' Variable? RelationshipTypes? (RangeLiteral)? Properties? ']'
Properties:           MapLiteral | Parameter
RelType:              ':' RelTypeName
RelationshipTypes:    ':' RelTypeName ('|' ':'? RelTypeName)*
NodeLabels:           NodeLabel (NodeLabel)*
NodeLabel:            ':' LabelName
RangeLiteral:         '*' (Number? '..' Number?)?
RelationshipsPattern: NodePattern (PatternElementChain)+
ListComprehension:    '[' FilterExpression ('|' Expression)? ']'
PropertyLookup:       '.' (PropertyKeyName | PropertyKeyName)
MapLiteral:           '{' (MapLiteralEntry (',' MapLiteralEntry)*)? '}'
MapLiteralEntry:      PropertyKeyName ':' Expression
PropertyExpression:   Atom (PropertyLookup)+
\end{lstlisting}


==> results-and-contributions.tex <==
% !TeX spellcheck = en_GB
% !TeX encoding = UTF-8
\section{Results and Contributions}


==> table-compilation.tex <==
\setlength\extrarowheight{2.5pt}
\setlength\tabcolsep{3.6pt}
\begin{table}[htbp]
\begin{adjustbox}{center}
\begin{tabular}{|l|l|l|c|}
	\hline
	\multicolumn{2}{|l|}{ \bf Language construct } & \bf Relational algebra expression & \\\hline\hline

	%\hline
	\multicolumn{4}{|l|}{Vertices and patterns. \lstinline|<p>p</p>| denotes a pattern that contains a vertex \lstinline|<<v>>|.} \\\cline{2-4}

	& \lstinline+(<<v>>)+ & $\getvertices{v}{}$ & \mapping{getvertices} \\\cline{2-4}

	& \lstinline+(<<v>>:<<l1>>:...:<<ln>>)+ & $\getvertices{v}{l1 \land \cdots \land ln}$ & \mapping{getverticeslabels} \\\cline{2-4}

	& \lstinline+<p>p</p>-[<<e>>:<<t1>>|...|<<tk>>]->(<<w>>)+ & $\expandout{v}{w}{}{e}{t1 \lor \cdots \lor tk}{1}{1} (p)$, where $e$ is an edge & \mapping{patterni} \\\cline{2-4}

	& \lstinline+<p>p</p><-[<<e>>:<<t1>>|...|<<tk>>]-(<<w>>)+ & $\expandin{v}{w}{}{e}{t1 \lor \cdots \lor tk}{1}{1} (p)$, where $e$ is an edge & \mapping{patternii} \\\cline{2-4}

	& \lstinline+<p>p</p><-[<<e>>:<<t1>>|...|<<tk>>]->(<<w>>)+ & $\expandboth{v}{w}{}{e}{t1 \lor \cdots \lor tk}{1}{1} (p)$, where $e$ is an edge & \mapping{patterniii} \\\cline{2-4}

	& \lstinline+<p>p</p>-[<<e>>*<<min>>..<<max>>]->(<<w>>)+ & $\expandout{v}{w}{}{e}{}{min}{max} (p)$, where $e$ is a list of edges& \mapping{patterniv} \\\cline{2-4}

	\hline \multicolumn{3}{|l|}{Combining and filtering pattern matches} & \\\cline{2-4}

	& \lstinline+MATCH <p>p1</p>, <p>p2</p>, ...+ &
	$\alldifferent{\atom{edges\ of\ p1,\ p2,\ \cdots}} \left( p1 \join p2 \join \cdots \right)$ & \mapping{matchi} \\\cline{2-4}

	& \breakable{
		\lstinline+MATCH <p>p1</p>+ \\
		\lstinline+MATCH <p>p2</p>+
	} &
	$\alldifferent{\atom{edges\ of\ p1}} \left(p1\right) \ \join\ \alldifferent{\atom{edges\ of\ p2}} \left(p2\right)$ & \mapping{matchii} \\\cline{2-4}

	& \breakable{
		\lstinline+OPTIONAL MATCH <p>p</p>+
	} & $ \{\tuple{}\} \ \leftouterjoin\ \alldifferent{\atom{edges\ of\ p}} \left(p\right)$ & \mapping{optionalmatchi} \\\cline{2-4}

	& \breakable{
		\lstinline+OPTIONAL MATCH <p>p</p> WHERE <p>condition</p>+
	} & $ \{\tuple{}\} \ \leftouterjoin_{\atom{condition}}\ \alldifferent{\atom{edges\ of\ p}} \left(p\right)$ & \mapping{optionalmatchwherei} \\\cline{2-4}

	& \breakable{
		\lstinline+[[r]] OPTIONAL MATCH <p>p</p>+
	} & $r \ \leftouterjoin\ \alldifferent{\atom{edges\ of\ p}} \left(p\right)$ & \mapping{optionalmatchii} \\\cline{2-4}

	& \breakable{
		\lstinline+[[r]] WHERE <<condition>>+
	} & \breakable{$\selection{\atom{condition}}{\left( r \right)}$} & \mapping{wherei} \\\cline{2-4}

	& \breakable{
		\lstinline+[[r]] WHERE (<<v>>:<<l1>>:...:<<ln>>)+ \\
	} & \breakable{$\selection{\var{l1} \in \vertexlabelfunction(v) \land \cdots \land \var{ln} \in \vertexlabelfunction(v)} (r) $ } & \mapping{whereii} \\\cline{2-4}	

	& \breakable{
		\lstinline+[[r]] WHERE <p>p</p>+ \\
	} & \breakable{$ r \join p $ } & \mapping{whereiii} \\\cline{2-4}

	%& \breakable{
	%	\lstinline+[[r]] WHERE NOT <p>p</p>+ \\
	%} & \breakable{$ r \antijoin p $ } & \mapping{whereiv} \\\cline{2-4}

	\hline \multicolumn{4}{|l|}{Result and subresult operations. Rules for \lstinline+RETURN+ also apply to \lstinline+WITH+.} \\\cline{2-4}

	& \lstinline+[[r]] RETURN <<x1>> AS <<y1>>, ...+ & $\projection{\var{x1} \assign \var{y1}, \cdots}{} \left( r \right)$ & \mapping{returni} \\\cline{2-4}

	& \lstinline+[[r]] RETURN DISTINCT <<x1>> AS <<y1>>, ...+ & $\duplicateelimination\left(\projection{\var{x1} \assign \var{y1}, \cdots}{} \left( r \right)\right)$ & \mapping{returnii} \\\cline{2-4}

	& \lstinline+[[r]] RETURN <<x1>>, <<aggr>>(<<x2>>)+ & $\grouping{\var{x1}, \atom{aggr}(\var{x2})}{\var{x1}}{\left( r \right)}$ (see \autoref{sec:aggregation}) & \mapping{returniii} \\\cline{2-4}

	& \breakable{
		\lstinline+[[r]] WITH <<x1>>+ \\
		\lstinline+[[s]] RETURN <<x2>>+
	} & \breakable{$\projection{\var{x2}}{}\Big(\big(\projection{\var{x1}}{} \left( r \right) \big) \join s\Big)$ } & \mapping{returniv} \\\cline{2-4}

	\hline \multicolumn{4}{|l|}{Unwinding and list operations} \\\cline{2-4}

	& \lstinline+[[r]] UNWIND <<xs>> AS <<x>>+ & $\unwind{\var{xs} \assign \var{x}}{\left( r \right)}$ & \mapping{unwind} \\\cline{2-4}

	& \lstinline+[[r]] ORDER BY <<x1>> ASC, <<x2>> DESC, ...+ & $\sort{\asc \var{x1}, \desc \var{x2}, \cdots}{\left( r \right)}$ & \mapping{orderby} \\\cline{2-4}

	& \lstinline+[[r]] SKIP <<s>> LIMIT <<l>>+ & $\topp{\var{l}}{\var{s}}(r)$
	& \mapping{top} \\\cline{2-4}

	\hline \multicolumn{4}{|l|}{Combining results } \\\cline{2-4}

	& \lstinline+[[r]] UNION [[s]] + & $r \union s$ & \mapping{union} \\\cline{2-4}

	& \lstinline+[[r]] UNION ALL [[s]] + & $r \bagunion s$ & \mapping{unionall} \\\hline
\end{tabular}
\end{adjustbox}
\caption{Mapping from \opencypher constructs to relational algebra. Variables, labels, types and literals are typeset as \lstinline|<<v>>|. The notation \lstinline|<p>p</p>| represents patterns resulting in a relation $p$, while \lstinline|[[r]]| denotes previous query fragment resulting in a relation $r$. To avoid confusion with the ``\lstinline+..+'' language construct (used for ranges), we use \lstinline+...+ to denote omitted query fragments.}
\label{table:mapping}
\end{table}


==> table-operators.tex <==
\setlength\tabcolsep{3.6pt}
\begin{table}[htbp]
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\multirow{1}{*}{\bf \#} &            \multirow{1}{*}{\bf notation}             & \multirow{1}{*}{\bf name} & \multirow{1}{*}{\bf schema} &  \\ \hline\hline
		\multirow{1}{*}{\bf 0}  &                 $\getvertices{v}{L}$                 &     \getverticestext      &                        $\tuple{\var{v}}$                         \\ \hline\hline
		\multirow{9}{*}{\bf 1}  &        $\expandboth{v}{w}{L}{e}{T}{1}{1} (r)$        &      \expandbothtext      &          $\schema{r} \append \tuple{\var{e}, \var{w}}$           \\ \cline{2-5}
%		                        &       $\unwind{\var{xs} \assign \var{x}} (r)$        &        \unwindtext        &  $\schema{r} \remove \tuple{\var{xs}} \append \tuple{\var{x}} $  \\ \cline{2-5}
%		                        &              $\nest{xs \assign x} (r)$               &         \nesttext         & $\schema{r} \remove \tuple{\atom{x}} \append \tuple{\atom{xs}} $ \\ \cline{2-5}
%		                        &             $\unnest{xs \assign x} (r)$              &        \unnesttext        & $\schema{r} \remove \tuple{\atom{xs}} \append \tuple{\atom{x}} $ \\ \hline\hline
		                        &          $\selection{\atom{condition}} (r)$          &      \selectiontext       &                           $\schema{r}$                           \\ \cline{2-5}
		                        &  $\projection{\var{x_1}, \var{x_2}, \ldots}{} (r)$   &      \projectiontext      &              $\tuple{\var{x_1}, \var{x_2}, \ldots}$              \\ \cline{2-5}
		                        &            $\duplicateeliminationop (r)$             & \duplicateeliminationtext &                           $\schema{r}$                           \\ \cline{2-5}
		                        & $\sort{\desc \var{x_1}, \asc \var{x_2}, \ldots} (r)$ &         \sorttext         &                           $\schema{r}$                           \\ \cline{2-5}
		                        &        $\topp{\atom{skip}}{\atom{limit}} (r)$        &         \toptext          &                           $\schema{r}$                           \\ \hline\hline
%		\multirow{4}{*}{\bf 2}  &                    $r \unionop s$                    &        \uniontext         &                           $\schema{r}$                           \\ \cline{2-5}
%		                        &                   $r \bagunion s$                    &       \baguniontext       &                           $\schema{r}$                           \\ \cline{2-5}
		                        &                    $r \joinop s$                     &         \jointext         &      $\schema{r} \append (\schema{s} \remove \schema{r}) $       \\ \cline{2-5}
%		                        &                 $r \leftouterjoin s$                 &    \leftouterjointext     &      $\schema{r} \append (\schema{s} \remove \schema{r}) $       \\ \cline{1-5}
		           %            &                  $r \antijoinop s$                   &          \antext          &                           $\schema{r}$                           \\ \cline{1-5}
	\end{tabular}
	\caption{Number of operands, properties and result schemas of relational graph algebra operators. For schema transformations, append is denoted by $\append$, while removal is marked by $\remove$. $L$ represents a (possibly empty) set of vertex labels and $T$ represents a (possibly empty) set of edge types.}
\label{table:operators}
\end{table}

